Skip-Attention: Improving Vision Transformers by Paying Less Attention

This work aims to improve the efficiency of vision transformers (ViT). While ViTs use computationally expensive self-attention operations in every layer, we identify that these operations are highly correlated across layers -- a key redundancy that causes unnecessary computations. Based on this observation, we propose SkipAt, a method to reuse self-attention computation from preceding layers to approximate attention at one or more subsequent layers. To ensure that reusing self-attention blocks across layers does not degrade the performance, we introduce a simple parametric function, which outperforms the baseline transformer's performance while running computationally faster. We show the effectiveness of our method in image classification and self-supervised learning on ImageNet-1K, semantic segmentation on ADE20K, image denoising on SIDD, and video denoising on DAVIS. We achieve improved throughput at the same-or-higher accuracy levels in all these tasks.

==> plots/plot_SSL.tex <==
% \begin{figure}
% \centering
% \setlength{\tabcolsep}{3pt}
% {\scriptsize\ref*{named_cifar}}
% \begin{tikzpicture}
% \begin{axis}[
% 	width=6.1cm,
% 	height=5cm,
% 	font=\scriptsize,
% 	xlabel={time/epoch},
% 	ylabel={top-1 accuracy (\%)},
% 	enlarge x limits=false,
% 	ymin=59.0, ymax=75,
% 	xtick={0,...,4},
% 	xticklabels={$20$,$40$,$60$, $80$, $100$},
% 	legend columns=3,
% % 	legend align = center
% 	legend to name=named_cifar,
% ]
% 	\pgfplotstableread{
% 		x    acc-d acc-ap  acc-sp
% 		0    59.4  60.8    59.7
% 		1    64.2  67.3    65.6
% 		2    69.4  71.2    70.8
% 		3    72.2  73.3    73.3
% 		4    73.6  74.1    73.9
% 	}{\ssl}
% 	\addplot[orange,mark=*, line width=1.3pt] table[y=acc-d]        {\ssl}; \leg{DINO}
% 	\addplot[ForestGreen,mark=*, line width=1.3pt] table[y=acc-ap] {\ssl}; \leg{DINO $+$ ~\methodabbrev}
% % 	\addplot[blue,mark=*, line width=1.3pt] table[y=acc-sp] {\ssl}; \leg{DINO $+$ SP}
	
% \end{axis}
% \end{tikzpicture}

% \caption{DINO \vs Ours \YA{perhaps the plot against training time is even better? (we can write in caption that both train for 100epochs}}
% % \vspace{-6pt}
% \label{fig:SSL}
% \end{figure}


\begin{figure}
\centering
\setlength{\tabcolsep}{3pt}
% {\scriptsize\ref*{named_cifar}}
\begin{tikzpicture}
\begin{axis}[
	title={},
	xlabel={time (in GPU-hours)},
	ylabel={top-1 accuracy (in \%)},
	width=6cm, height=5cm,
	xmin=23, xmax=132,
	ymin=59, ymax=75,
	legend pos=south east,
	legend columns=1,
	ymajorgrids=true,
	grid,
]
	\addplot[red,mark=*]coordinates {
		(26,59.4)(52.4, 64.2)(78.6, 69.4)(104.8, 72.2)(131, 73.6)
		}; \leg{DINO}
	\addplot[blue,mark=*]coordinates {
		(24,60.8)(48, 67.3)(72, 71.2)(96, 73.3)(120, 74.1)
		}; \leg{DINO $+$ \methodabbrev}
\end{axis}
\end{tikzpicture}

\caption{\tb{Self}
}
%\YA{perhaps the plot against training time is even better? (we can write in caption that both train for 100epochs}
%\ag{add caption for the figure. why in the horizontal axis we have time/epoch?   } 
\YA{it should just be time, so maybe make it in GPU-hours} \YA{this figure could also be even thinner, as it doesn't have huge amount of info.
\ag{a horizontal arrow to show when top-1 acc reaches to the baseline could be informative}}
\vspace{-6pt}
\label{fig:SSL}
\end{figure}

==> plots/plot_ade.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\linewidth]{figs/ade20k_fps.png}
\includegraphics[width=0.48\linewidth]{figs/ade20k_flops.png}
\caption{Performance comparison of baseline ViT~\cite{} and Ours wrt throughput (left) and FLOPs (Right). \ag{update the numbers for stacked model}  }
\label{fig:ade20k}
\vspace*{-5mm}
\end{figure}

==> plots/plot_sidd.tex <==
\begin{figure}
\centering
\setlength{\tabcolsep}{3pt}
% {\scriptsize\ref*{named_cifar}}
\begin{tikzpicture}
\begin{axis}[
	title={},
	xlabel={GFLOPs},
	ylabel={PSNR (in dB)},
	width=7cm, height=5cm,
% 	width=8cm, height=5cm,
	xmin=10, xmax=100,
	ymin=39.64, ymax=39.95,
	legend pos=south east,
	legend columns=1,
	ymajorgrids=true,
	grid,
]
	\addplot[red,mark=*]coordinates {
		(12,39.66)(44, 39.77)(89, 39.89)
		}; \leg{Uformer}
	\addplot[blue,mark=*]coordinates {
		(11,39.69)(39, 39.84)(77, 39.94)
		}; \leg{Uformer $+$ AP}
\end{axis}
\end{tikzpicture}

\caption{\emph{PSNR \vs GFLOPs} on SIDD for image denoising. \alert{add points of other methods too} }
% \vspace{-6pt}
\label{fig:sidd-denoising}
\end{figure}

==> tables/sota_imagenet-1.tex <==
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llcccc} \toprule
 \Th{Backbone}    & \Th{Method}                             &\Th{top-1}   & \Th{Param}        & \Th{GFlops}   & \Th{Throughput}          \\ 
                  &                                         & (\%)        & ($\times 10^6$)   &               & (img/sec $\times 10^3$)  \\ \midrule
                  & ViT~\cite{dosovitskiy2020image}         & 72.8        & 5.7               & 1.2           & 5.5                      \\
                  & A-ViT~\cite{yin2022vit}                 & 71.0        & 5.7               & 0.8           &                          \\
ViT-T/16          & Dynamic ViT~\cite{rao2021dynamicvit}    & 70.9        & --                & 0.9           &                          \\
                  & SViTE~\cite{chen2021chasing}            & 71.7        & 4.0               & 0.9           &                          \\
                  & ConvNeXt (iso)~\cite{liu2022convnet}    & 72.7        & 5.7               & 1.1           & 5.8                      \\
                  & SPViT~\cite{kong2021spvit}              & 72.7        & 5.7               & 0.9           & 6.7                      \\
                  & ATS~\cite{fayyazadaptive}               & 72.7        & 5.7               & 0.9           & 6.1                      \\
                  & PS-ViT~\cite{tang2022patch}             & 72.6        & --                & 0.7           & 7.1                      \\
                  & HVT~\cite{pan2021scalable}              & 70.2        & 5.7               & 0.7           &                          \\
                  %
                  \cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}
                  & PVT-v2-B1                               & 78.7        & 13.1              & 2.1           &                          \\
                  & PVT-v1-Tiny                             & 75.1        & 13.2              & 1.9           &                          \\
                  & T2T-ViT~\cite{yuan2021tokens}           & 71.7        & 5.8               & 1.1           &                          \\
                  & LeViT-256~\cite{graham2021levit}        & 81.2        & 18.9              & 1.1           &                          \\
                  & EdgeViT-XS                              & 77.5        & 6.7              & 1.1           &                           \\
                  & EdgeViT-XXS                             & 74.4        & 4.1              & 0.6           &                           \\
                  & Mobileformer-294                        & 77.9        & 11.8              & 0.3           &                          \\
                  \cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}
                  %
                  \rowcolor{}& Alternate param $\times 1$              & 73.6        & 5.4               & 1.14          & 7.0                      \\
                  & Alternate param $\times 2$              & 74.0        & 5.7               & 1.16          & 6.7                      \\ 
                  & Stacked param $\times 1$                & 72.6        & 5.3               & 1.08          & 7.4                      \\
                  & Stacked param $\times 2$                & 72.9        & 5.8               & 1.14          & 6.8                      \\
                  \midrule 
                  %----------------------------------------------------------------------------------------------------------------------------------------------------------------
                  & ConvNext-T                              & 82.1        & 29.0              & 4.5           & 2.6                      \\
                  & ConvNeXt (iso)~\cite{liu2022convnet}    & 79.7        & 22.4              & 4.3           & 3.3                      \\
                  & Swin-T                                  & 81.3        & 28.3              & 4.5           & 2.5                      \\
                  %
                  \cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}
                 %   & T2T-ViT~\cite{yuan2021tokens}           & 80.7        & 21.5              & 5.2           &                          \\
                  & CMT-S                                   & 83.5        & 25.0              & 4.0           &                           \\  
                  & CoaT-Lite-Small                         & 81.9        & 20.0              & 4.0           &                          \\
                  & PVT-v2-B2-Li                            & 82.1        & 22.6              & 3.9           &                           \\
                  & PVT-v1-Small                            & 79.8        & 24.5              & 3.8           &                           \\
                  & Poolformer-S24                          & 80.3        & 21.0              & 3.4           &                       \\
                  & Twins-SVT-S                             & 81.7        & 24.0              & 2.8           &                           \\
                  & LeViT-384~\cite{graham2021levit}        & 82.6        & 39.1              & 2.3           &                       \\
                  & MobileViT-S                             & 78.4        & 5.6              & 2.0           &                       \\
                  & EdgeViT-S                               & 81.0        & 11.1              & 1.9           &                       \\
                  \cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}
                  %
                  & ViT~\cite{dosovitskiy2020image}         & 79.8        & 22.4              & 4.6           & 3.2                      \\
                  & A-ViT~\cite{yin2022vit}                 & 78.6        & 22.4              & 3.6           & 3.4                      \\
                  & Dynamic ViT~\cite{rao2021dynamicvit}    & 78.3        &                   & 3.4           & 3.6                      \\
                  & PVT~\cite{wang2021pyramid}              & 79.8        & 24.5              & 3.8           &                          \\
ViT-S/16          & SViTE~\cite{chen2021chasing}            & 80.2        & 13.1              & 2.7           & 3.5                      \\
                  & ATS~\cite{fayyazadaptive}               & 79.7        & 22.4              & 2.9           & 3.6                      \\
                  & PS-ViT~\cite{tang2022patch}             & 79.4        & --                & 2.6           & 4.1                      \\
                  
                  & SPViT~\cite{kong2021spvit}              & 72.3        & 22.1              & 2.7           &                          \\
                  & HVT\cite{pan2021scalable}               & 78.0        & 22.5              & 2.4           &                          \\
                  \cmidrule{2-6}
                  & Alternate param $\times 1$              & 79.3        & 20.9              & 4.1           & 3.8                      \\
                  & Alternate param $\times 2$              & 79.6        & 22.1              & 4.2           & 3.7                      \\
                  & Stacked param $\times 1$                & 79.5        & 20.3              & 4.1           & 3.9                      \\ 
                  & Stacked param $\times 2$                & 80.2        & 22.1              & 4.0           & 3.5                      \\
                  %----------------------------------------------------------------------------------------------------------------------------------------------------------------
                  \midrule
                  & ViT~\cite{dosovitskiy2020image}         & 81.8        & 87.3              & 17.6          & 1.2                      \\
                  & PVT~\cite{wang2021pyramid}              & 81.7        & 61.4              & 9.8           &                          \\
                  & SViTE~\cite{chen2021chasing}            & 81.6        & 52.0              & 11.5          &                          \\
                  & ConvNext-B                              & 83.0        & 89.0              & 15.4          & 1.1                      \\
ViT-B/16          & ConvNeXt (iso)~\cite{liu2022convnet}    & 82.0        & 87.3              & 16.9          & 1.3                      \\
                  & PS-ViT~\cite{tang2022patch}             & 81.5        &  --               & 9.8           &                          \\
                  & Swin-S                                  & 83.5        & 88.0              & 15.4          & 1.0                      \\
                  %
                  \cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}
                  & Twins-SVT-B                             & 83.2        & 56.0              & 8.6           &                           \\
                  \cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}\cmidrule{2-6}
                  %
                  \cmidrule{2-6}
                  & Alternate param $\times 1$              &             & 81.9              & 14.2          & 1.5                      \\
                  & Alternate param $\times 2$              &             & 86.7              & 15.4          & 1.4                      \\
                  & Stacked param $\times 1$                &             & 79.5              & 13.8          & 1.6                      \\
                  & Stacked param $\times 2$                &             & 86.7              & 15.2          & 1.4                       \\
                  \bottomrule
\end{tabular}
\label{table:sota-imagenet}
\end{table}


==> text/analysis.tex <==
% \section{Analysis}
% \label{sec:ananlysis}


% Visualizing self-attentions across blocks and show the correlations (maybe against random images)
